Achievable Information Rates for Fiber Optics: Applications and Computations

In this paper, achievable information rates (AIR) for fiber optical communications are discussed. It is shown that AIRs such as the mutual information and generalized mutual information are good design metrics for coded optical systems. The theoretical predictions of AIRs are compared to the performance of modern codes including low-parity density check (LDPC) and polar codes. Two different computation methods for these AIRs are also discussed: Monte-Carlo integration and Gauss-Hermite quadrature. Closed-form ready-to-use approximations for such computations are provided for arbitrary constellations and the multidimensional AWGN channel. The computation of AIRs in optical experiments and simulations is also discussed.

==> vfinal arxiv/myFigures.tex <==
%% figure definitions

%% default
\usetikzlibrary{plotmarks,matrix,chains,scopes,fit,calc,shapes,positioning,decorations,intersections,arrows,backgrounds,shadows}
% \pgfplotsset{compat=1.15}
%\pgfplotsset{compat=newest} 
%\pgfplotsset{plot coordinates/math parser=false}
% \graphicspath{{Figures/}}


%% line styles
%\pgfplotsset{every axis/.append style={font=\footnotesize}}
%\pgfplotsset{every axis legend/.append style={font=\footnotesize, legend cell align=left,at={(0.02,0.98)},anchor=north west}}
%\pgfplotsset{every axis plot/.append style={line width=1.5pt}} % lines
%\pgfplotsset{every axis plot/.append style={mark options={solid,fill=white!80!.,line width=0.5pt},mark size = 2.5pt}} % mark


% figure dimensions
\newlength\FigureHeight
\newlength\FigureWidth
\setlength\FigureWidth{1.03\columnwidth}
\setlength\FigureHeight{.77\columnwidth}


%% tikz externalize
% \usepgfplotslibrary{external} 
% \tikzexternalize[prefix=./tikz/]


\newcommand{\inputtikz}[1] {% directly input tikz without tikzscale
% \tikzsetnextfilename{#1}%
 \input{./figures/#1.tikz}
}



==> vfinal arxiv/myMacros.tex <==
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\ASE}{\ensuremath{\sigma^2_{\text{ASE}}}\xspace}
\newcommand{\SNR}{\ensuremath{\text{SNR}_{\text{eff}}}\xspace}

\newcommand{\changed}[1]{\textcolor{red}{#1}}

\newcounter{lemma}
\newtheorem{theorem}[lemma]{Theorem}
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{exampleplain}{Example}
\newtheorem{remark}{Remark}
\newenvironment{example}{\begin{exampleplain}}{~\hfill$\vartriangle$\end{exampleplain}}

% Commands from tutorial
\newcommand{\cd}{\cdot}
\newcommand{\mcIkb}{\mathcal{I}_{k}^{b}}
%\newcommand{\mcXko}{\mathcal{X}_{k}^{1}}
%\newcommand{\mcXkz}{\mathcal{X}_{k}^{0}}
%\newcommand{\Es}{\sigma_x^2}
\newcommand{\dij}[0]{d_{ij}}\newcommand{\bdij}[0]{\boldsymbol{d}_{ij}}
\newcommand{\dil}[0]{d_{il}}\newcommand{\bdil}[0]{\boldsymbol{d}_{il}}
\newcommand{\dip}[0]{d_{ip}}\newcommand{\bdip}[0]{\boldsymbol{d}_{ip}}



%% Commands from Old JLT
\newcommand{\set}[1]{\{#1\}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\secref}[1]{Sec.~\ref{#1}}
\newcommand{\figsref}[2]{Figs.~\ref{#1} and \ref{#2}}
\newcommand{\tr}[1]{\mathrm{#1}}
\newcommand{\ld}{\ldots}
\newcommand{\ms}[1]{\mathds{#1}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bC}{\boldsymbol{C}}\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bB}{\boldsymbol{B}}\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bX}{\boldsymbol{X}}\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bR}{\boldsymbol{R}}\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bY}{\boldsymbol{Y}}\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bZ}{\boldsymbol{Z}}\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bU}{\boldsymbol{U}}\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bS}{\boldsymbol{S}}\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bL}{\boldsymbol{L}}\newcommand{\bl}{\boldsymbol{l}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\mcC}{\mathcal{C}}
\newcommand{\mcB}{\mathcal{B}}
\newcommand{\mcX}{\mathcal{X}}
\newcommand{\mcS}{\mathcal{S}}
\newcommand{\mcH}{\mathcal{H}}
\newcommand{\mcV}{\mathcal{V}}
\newcommand{\mcXkb}{\mathcal{X}_{k}^{b}}
\newcommand{\mcXko}{\mathcal{X}_{k}^{1}}
\newcommand{\mcXkz}{\mathcal{X}_{k}^{0}}
%\newcommand{\Real}{\mathbb{R}}
\newcommand{\Ns}{L}
\newcommand{\MCs}{D}
\newcommand{\GHs}{J}
\newcommand{\Nspan}{N_{\tnr{s}}}
\newcommand{\Es}{E_\tr{s}}
\newcommand{\Rs}{R_\tr{s}}
\newcommand{\Rc}{R_\tr{c}}
\newcommand{\Ex}{\ms{E}}
\newcommand{\R}{R}
\newcommand{\ov}[1]{\overline{#1}}
\newcommand{\un}[1]{\underline{#1}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
%\newcommand{\argmax}{\mathop{\mathrm{argmax}}}

%% Fiber Setup
\newcommand{\Nch}{\ensuremath{N_{\text{ch}}}\xspace}
\newcommand{\Bch}{\ensuremath{B_{\text{ch}}}\xspace}
\newcommand{\Nspans}{\ensuremath{N_{\text{spans}}}\xspace}

%% Operators
\newcommand{\E}{\ensuremath{\mathbb{E}}}
\newcommand{\I}{\ensuremath{\mathbb{I}}}
\newcommand{\Entr}{\ensuremath{\mathbb{H}}}
\newcommand{\entr}{\ensuremath{\mathbb{h}}}
\newcommand{\Real}[1]{\mathbb{R}\{#1\}}
\newcommand{\Imag}[1]{\mathbb{I}\{#1\}}


%% AIR
\newcommand{\Rbmd}{\ensuremath{\text{R}_{\text{BMD}}}\xspace}
\newcommand{\Ibmdhat}{\ensuremath{\hat{I}_{\text{BMD}}}\xspace}

%\newcommand{\GMI}{\ensuremath{\text{G}}\xspace}
%\newcommand{\MI}{\ensuremath{\text{M}}\xspace}
\newcommand{\GMI}{\ensuremath{G}\xspace}
\newcommand{\MI}{\ensuremath{I}\xspace}

\newcommand{\LLR}{\ensuremath{\text{LLR}}}
\newcommand{\Rsym}{\ensuremath{\text{R}_{\text{SYM}}}\xspace}
\newcommand{\Rsymhat}{\ensuremath{\hat{\text{R}}_{\text{sym}}}\xspace}

%% RVs
\newcommand{\X}{\ensuremath{X}\xspace}
\newcommand{\Xn}{\ensuremath{X^n}\xspace}
\newcommand{\Y}{\ensuremath{Y}\xspace}
\newcommand{\Yn}{\ensuremath{Y^n}\xspace}
\newcommand{\B}{\ensuremath{\boldsymbol{B}}\xspace}
\newcommand{\setX}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\x}{\ensuremath{x}\xspace}
\newcommand{\y}{\ensuremath{y}\xspace}

\newcommand{\kth}{\ensuremath{k^{\text{th}}}\xspace}
\newcommand{\auxch}{\ensuremath{q_{\Y|\X}}\xspace}

%% SNR
\newcommand{\Ptx}{\ensuremath{P_{\text{tx}}}\xspace}
\newcommand{\Ptxopt}{\ensuremath{P_{\text{tx,opt}}}\xspace}
\newcommand{\sigmaASE}{\ensuremath{\sigma^2_{\text{ASE}}}\xspace}
\newcommand{\NoiseEff}{\ensuremath{\sigma^2_{\text{eff}}}\xspace}
\newcommand{\SNREff}{\ensuremath{\text{SNR}_{\text{eff}}}\xspace}
\newcommand{\NoiseNLI}{\ensuremath{\sigma^2_{\text{NLI}}}\xspace}
\newcommand{\NoiseIntra}{\ensuremath{\sigma^2_{\text{NLI,intra}}}\xspace}
\newcommand{\NoiseInter}{\ensuremath{\sigma^2_{\text{NLI,inter}}}\xspace}
\newcommand{\EbN}{\ensuremath{E_\text{b}/N_0}\xspace}
\newcommand{\EsN}{\ensuremath{E_\text{s}/N_0}\xspace}


%% short notation
\newcommand{\tento}[1]{$\times$10\textsuperscript{#1}}
\newcommand{\tnr}[1]{{\textnormal{#1}}}


%%
\newcommand{\BERin}{\ensuremath{\text{BER}_{\text{in}}}\xspace}
\newcommand{\BERout}{\ensuremath{\text{BER}_{\text{out}}}\xspace}
\newcommand{\RSD}{\ensuremath{\text{R}_{\text{SD}}}\xspace}
\newcommand{\RHD}{\ensuremath{\text{R}_{\text{HD}}^1}\xspace}
\newcommand{\RHDm}{\ensuremath{\text{R}_{\text{HD}}^{m}}\xspace}
\newcommand{\RHDone}{\ensuremath{\text{R}_{\text{HD}}^1}\xspace}
\newcommand{\gammaeff}{\ensuremath{\gamma_\text{eff}}\xspace}

%% units
\newcommand{\unitgamma}{\ensuremath{\frac{1}{\text{W} \cdot \text{km}}}\xspace}

%% Comments
\newcommand{\todo}[1]{\textcolor{magenta}{\uline{#1}}}
\newcommand{\tf}[1]{\textcolor{red}{\uline{#1}}}
\renewcommand{\aa}[1]{\textcolor{blue}{\uline{#1}}}

==> vfinal arxiv/myPackages.tex <==
\usepackage[utf8]{inputenc}

%% Math
\usepackage{amsmath,amssymb}

%% Graphics
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{float}
\usepackage{balance}

%% Div
\usepackage{xspace}
\usepackage[normalem]{ulem}
\usepackage[pdftex]{hyperref} %pdflatex
\hypersetup{colorlinks,linkcolor=red,citecolor=blue} % hyperref colors

\usepackage{dsfont,empheq}
\usepackage{multicol,multirow}

\usepackage{cite}

==> vfinal arxiv/myStyles.tex <==
%% defaults
\pgfkeys{/pgf/number format/.cd,1000 sep={}}
\pgfplotsset{every axis legend/.append style={legend cell align=left,at={(0.02,0.97)},anchor=north west}}
\pgfplotsset{every axis plot/.append style={line width=1.5pt}} % lines
\pgfplotsset{every axis plot/.append style={mark options={solid,fill=white!80!.,line width=0.5pt},mark size = 3pt}} % mark

% colors
\definecolor{myDarkGreen}{rgb}{0.00000,0.58824,0.00000}%
\definecolor{uniform}{rgb}{0.00000,0.58824,0.00000}%
\definecolor{matched}{rgb}{1,0.58824,0.00000}%
\definecolor{mismatched}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{AWGNreference}{rgb}{0.00000,0.58824,0.00000}%
\definecolor{XPMmodel}{rgb}{0,0,0}%
\definecolor{sims}{rgb}{0.00000,0.44700,0.74100}%


%% my plot styles
\pgfplotsset{AWGN_capacity/.style={color=gray,dotted}}
\pgfplotsset{16QAM_uniform/.style={color=blue,dashed}}
\pgfplotsset{16QAM_shaped/.style={color=blue,solid}}
\pgfplotsset{64QAM_uniform/.style={color=red,dashed}}
\pgfplotsset{64QAM_shaped/.style={color=red,solid}}
\pgfplotsset{256QAM_uniform/.style={color=brown,dashed}}
\pgfplotsset{256QAM_shaped/.style={color=brown,solid}}

\pgfplotsset{AWGNreference/.style={color=AWGNreference,dotted}}
\pgfplotsset{XPMmodel/.style={color=XPMmodel,dashed}}
\pgfplotsset{sims/.style={color=sims,only marks,mark=*,mark options={solid,fill=white}}}
